Vector bundles on singular surfaces and threefolds

We fully classify vector bundles of critical rank on normal affine surfaces and threefolds over algebraically closed fields via their Chern classes. We also prove existence of rank $2$ bundles on threefolds with prescribed first and second motivic Chern classes. The main input is the motivic filtration on algebraic $K$-theory: its third piece is generated by smooth closed points and is identified with motivic cohomology by the third Chern class.

==> amsbib.sty.tex <==
%      â¨«¥¢®© ä ©« AMSBIB.STY ¤«ï ®ä®à¬«¥­¨ï á¯¨áª  «¨â¥à âãàë
%             ¢ LaTeX2¥ ¯®áà¥¤áâ¢®¬ AmS-TeX'®¢áª¨å ª®¬ ­¤
%
%                    ¤«ï LaTeX2e ¯®¤ MikTeX
%
%             ®á«¥¤­¥¥ ¨á¯à ¢«¥­¨¥ 16  ¢£ãáâ  2010
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\NeedsTeXFormat{LaTeX2e}[1995/12/01]

\newif\if@hyper
\@hypertrue
\newif\if@logos
\@logosfalse
\DeclareOption{hyper}{\@hypertrue\@logostrue}
\DeclareOption{logos}{\@logostrue}
\DeclareOption{dataonly}{\@logostrue}
\ProcessOptions

\RequirePackage{graphicx}

\newread\@@Read
\newwrite\@@Write


\let\z@Z=n


\def\bef@rall{%
\immediate\openin\@@Read=pdfs.txt \relax
\ifeof\@@Read \else\global\@hypertrue \fi
\immediate\closein\@@Read
\let\bef@rall\relax}


\bef@rall




\def\endthebibliography{\nobreak\@@par\def\@noitemerr{}\endlist}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    ªà®áë ¤«ï ®ä®à¬«¥­¨ï á¯¨áª  «¨â¥à âãàë:

\newcounter{aux@counter}

\def\thebibliography#1{%
\refstepcounter{aux@counter}%
\addcontentsline{toc}{section}{\refname}%
\section*{\refname}
\def\@biblabel##1{{\select@language{russian}[##1]}}
\small
\list
 {\@biblabel{\arabic{enumi}}}{\settowidth\labelwidth{\@biblabel{#1}}\leftmargin\labelwidth
 \advance\leftmargin\labelsep
 \usecounter{enumi}}
 \baselineskip3.8mm
 \parskip-0.5pt
 \def\newblock{\hskip .11em plus .33em minus .07em}
 \sloppy\clubpenalty4000\widowpenalty4000
 \sfcode`\.=1000\relax
 \def\makelabel##1{\hfil ##1}
}


\def\eat@#1{}

\newif\ifbook@
\newif\ifprocpaper@
\RequirePackage{color}

\def\nofrills{%
  \expandafter\ifx\envir@end\end@@ref
    \let\do\relax
    \xdef\nofrills@list{\nofrills@list\do\curbox}%
  \else\errmessage{\Invalid@@ \string\nofrills}%
  \fi}%

\newif\if@Ref@
\@Ref@false
\newif\ifmoreref@
\newif\if@kern

\def\test@Ref@{\if@Ref@\else\@@Ref\fi}

\def\@@Ref{\ifhmode\unskip\else\leavevmode\fi
  \begingroup \@Ref@true
  \def\envir@end{\end@@ref}%
  \let\par\end@@ref
  \global\let\nofrills@list\empty
  \refbreaks%
  \procpaper@false \book@false \moreref@false
  \def\curbox{\z@}\setbox\z@\vbox\bgroup
}
\let\keyhook@\empty


\def\jour@true{\global\book@false\global\procpaper@false}%


\newbox\translbox@
\newbox\holdoverbox
\newbox\bybox@

\gdef\page@text{\pagetext}%
\gdef\by{\makerefbox\bybox@{\empty\byfont}}
\gdef\with{\makerefbox\withbox@{\empty\withfont}} \newbox\withbox@
\let\manyby\by % for backward compatibility
\def\bysame{\by\hbox to3em{\hrulefill}\thinspace\kern\z@}%
\def\paper{\makerefbox\paperbox@\empty} \newbox\paperbox@
\def\paperinfo{\makerefbox\paperinfobox@\empty} \newbox\paperinfobox@
\gdef\jour{\makerefbox\jourbox@{\it\aftergroup\jour@true}}%
\newbox\jourbox@
\def\issue{\makerefbox\issuebox@\empty} \newbox\issuebox@
\def\yr{\makerefbox\yrbox@\empty} \newbox\yrbox@
\def\pages{\makerefbox\pagesbox@\empty} \newbox\pagesbox@
\def\page{\gdef\page@text{\pagestext}\makerefbox\pagesbox@\empty}%
\def\page{\makerefbox\pagesbox@\empty}%
\def\ed{\makerefbox\edbox@\empty} \newbox\edbox@
\def\eds{\ed}%
\def\book{\makerefbox\bookbox@{\it\aftergroup\book@true}}%
\newbox\bookbox@
\def\publ{\makerefbox\publbox@\empty} \newbox\publbox@
\def\publaddr{\makerefbox\publaddrbox@\empty} \newbox\publaddrbox@
\gdef\inbook{\makerefbox\bookbox@{\it\aftergroup\procpaper@true}}
\def\procinfo{\makerefbox\procinfobox@\empty} \newbox\procinfobox@
%\def\finalinfo{\makerefbox\finalinfobox@\empty} \newbox\finalinfobox@
%\def\@@finalinfo{\makerefbox\@@finalinfobox@\empty} \newbox\@@finalinfobox@
\def\miscnote{\makerefbox\miscnotebox@\empty} \newbox\miscnotebox@
\def\toappear{\miscnote \t@appear}%
\def\lang{\makerefbox\langbox@\empty} \newbox\langbox@
\def\vol{\makerefbox\volbox@{\bf}}%
\newbox\volbox@
\def\bookinfo{\makerefbox\bookinfobox@{\aftergroup\procpaper@true\rm}} \newbox\bookinfobox@
\def\serial{\makerefbox\serialbox@{\aftergroup\procpaper@true\rm}} \newbox\serialbox@

\def\misc@{\makerefbox\misc@box@\empty\ifx\cyrillicencoding\@undefined\else\select@language{russian}\fi} \newbox\misc@box@

\let\preprint=\book
\def\preprintinfo{\makerefbox\bookinfobox@{\aftergroup\book@true\rm
\let\@my@href=\href\relax\def\href##1##2{\@my@href{##1}{{\tt ##2}}}}}


\let\thesis=\preprint
\let\thesisinfo=\preprintinfo

\let\eprint=\preprint
\let\eprintinfo=\preprintinfo

\def\makerefbox#1#2{\test@Ref@\endgraf
  \setbox\z@\lastbox
  \global\setbox\@ne\hbox{\unhbox\holdoverbox
    \ifvoid\z@\else\unhbox\z@\unskip\unskip\unpenalty\fi}%
  \egroup
  \setbox\curbox\box\ifdim\wd\@ne>\z@ \@ne \else\voidb@x\fi
  \def\curbox{#1}\setbox#1\vbox\bgroup \hsize\maxdimen \noindent
  #2\leftskip0truemm\relax}


\def\refbreaks{%
\def\refconcat##1{\setbox\z@\lastbox \setbox\holdoverbox\hbox{%
\unhbox\holdoverbox \unhbox\z@\unskip\unskip\unpenalty##1}}%
\def\holdover##1{%
\RIfM@
%      Break the current line, adding \null to ensure proper spacing
%      for a preceding mathrel or mathbin.
\penalty -\@M\null
%      Put a temporary ending of the current math formula on the next
%      line, by itself.
\hfil$\clubpenalty\z@\widowpenalty\z@\interlinepenalty\z@
\offinterlineskip\endgraf
%      Now remove that unwanted extra line and the preceding \lineskip
%      (of 0pt) and any  penalty.  There shouldn't be any penalty,
%      actually, because the relevant penalties were set to 0 above;
%      but the \unpenalty is harmless and perhaps there is an
%      overlooked eventuality that it will catch.
\setbox\z@\lastbox\unskip \unpenalty
\refconcat{##1}%
\noindent
%      Since we did a temporary end of the current math formula there
%      remains some more math coming up; therefore we need to shift
%      into math mode again.  By breaking immediately after the
%      beginning of the math formula we leave the unwanted extra
%      \mathon item in a line by itself; this will be ignored because
%      in the unpacking process we will only take the last line out of
%      the current \vbox.
$\hfil\penalty -\@M
%      No \null here because we don't need to do anything extra to
%      affect the math spacing of the following item.
\else {\parfillskip0pt
\endgraf}\refconcat{##1}\noindent
\fi}%
\def\break{\holdover{\penalty -\@M}}%
\def\linebreak{\holdover{\penalty -\@M}}%
\def\newline{\holdover{\hfill\penalty -\@M}}%
\let\vadjust@\vadjust
\def\vadjust##1{\holdover{\vadjust@{##1}}}%
%      It seems unlikely that \newpage will be needed inside of a
%      \ref...\endref construction (more likely it will occur between
%      references, if at all).  So we provide only a very simple
%      alternate version using \vadjust.
\def\newpage{\vadjust{\vfill\break}}%
}%


\def\finalpunct{\ifnum\lastkern=\m@ne\unkern\else\if@finalpunct@.\fi\fi
       \refquotes@\refbreak@}%
\def\continuepunct#1#2#3#4{}%


\def\end@@ref{\makerefbox \z@ {\endgraf \egroup }\end@ref@ \endgraf \endgroup
\keyhook@ \global \let \keyhook@ \empty\color[rgb]{0,0,0}}

\def\end@ref@{%
\def\nofrillscheck##1{%
\def\do####1{\ifx##1####1\let\frills@\eat@\fi}%
\let\frills@\identity@ \nofrills@list}%
\@ref}


\gdef\@ref{%\spaceskip 0.5 emplus.5em minus0.2em%
%\tolerance1000%
\@kernfalse
\ifmoreref@
    \commaunbox@\translbox@
\else
    \@kerntrue
\fi
\if@kern\kern-\tw@ sp\kern\m@ne sp\fi \@@ref
\color[rgb]{0,0,0}}


\def\moreref{\transl}
\def\morerref{\rtransl}


\def\transl{%
\makerefbox\z@{\endgraf\egroup}%
\let\savedef@\finalpunct  \let\finalpunct\empty
\end@ref@
%\book@false\procpaper@false
\defaultreftexts
\def\punct@##1##2{\unskip ##2{\@No@Color;}\allowbreak\ }%
\global\let\nofrills@list\empty%
\let\finalpunct\savedef@
\moreref@true
\def\curbox{\translbox@}%
\setbox\translbox@\vbox\bgroup \hsize\maxdimen \noindent
\misc@\nofrills}%

\def\rtransl{%
\makerefbox\z@{\endgraf\egroup}%
\let\savedef@\finalpunct  \let\finalpunct\empty
\end@ref@
%\book@false\procpaper@false
\defaultrusreftexts
\def\punct@##1##2{\unskip ##2{\@No@Color;}\allowbreak\ }%
\global\let\nofrills@list\empty%
\let\finalpunct\savedef@
\moreref@true
\def\curbox{\translbox@}%
\setbox\translbox@\vbox\bgroup \hsize\maxdimen \noindent
\misc@\nofrills}%

\newif\if@misc@transl
\@misc@translfalse

\def\misctransl{%
\makerefbox\z@{\endgraf\egroup}%
\let\savedef@\finalpunct  %\let\finalpunct\empty
\def\finalpunct{\if@finalpunct@\@No@Color.\fi}%
\end@ref@
\defaultreftexts
\@misc@transltrue
\def\punct@##1##2{\unskip ##2{\@No@Color}\allowbreak\
\if@misc@transl[\kern-\spaceskip\nobreak\fi
}%
\global\let\nofrills@list\empty%
\let\finalpunct\savedef@
\moreref@true
\def\curbox{\translbox@}%
\setbox\translbox@\vbox\bgroup \hsize\maxdimen \noindent
\misc@}%

\def\miscrtransl{%
\makerefbox\z@{\endgraf\egroup}%
\let\savedef@\finalpunct  %\let\finalpunct\empty
\def\finalpunct{\if@finalpunct@\@No@Color.\fi}%
\end@ref@
\defaultrusreftexts
\@misc@transltrue
\def\punct@##1##2{\unskip ##2{\@No@Color}\allowbreak\
\if@misc@transl[\kern-\spaceskip\nobreak\fi
}%
\global\let\nofrills@list\empty%
\let\finalpunct\savedef@
\moreref@true
\def\curbox{\translbox@}%
\setbox\translbox@\vbox\bgroup \hsize\maxdimen \noindent
\misc@}%



%
\def\punct@#1{#1}
\def\ppunbox@#1#2#3#4{\ifvoid#3\else
  \let\prespace@\relax
  \ifnum\lastkern=\m@ne \unkern\let\punct@\eat@
    \ifnum\lastkern=-\tw@ \unkern\let\prespace@\ignorespaces \fi
  \fi
  \nofrillscheck#3%
  \punct@{#1}\refquotes@\refbreak@
  \let\punct@\identity@
  \prespace@
  \frills@{#2\eat@}\space
  \unhbox#3\breakcheck
  \frills@{#4\eat@}{\kern\m@ne sp}\fi}

\def\commaunbox@#1{\ppunbox@,\space{#1}\empty}

\def\pnktunbox@#1{\ppunbox@.\space{#1}\empty}%


\def\breakcheck{\edef\refbreak@{\ifnum\lastpenalty=\z@\else
  \penalty\the\lastpenalty\relax\fi}\unpenalty}
\def\endquotes{\def\refquotes@{''\let\refquotes@\empty}}
\let\refquotes@\empty
\let\refbreak@\empty



\def\identity@#1{#1}
\def\nofrills@@#1{%
 \DN@{#1}%
 \ifx\next\nofrills \let\frills@\eat@
   \expandafter\expandafter\expandafter\next@\expandafter\eat@
  \else \let\frills@\identity@\expandafter\next@\fi}

\def\nofrillscheck#1{\def\nofrills@{\nofrills@@{#1}}%
  \futurelet\next\nofrills@}

\def\add@missing#1{\expandafter\ifx\envir@end#1%
  \Err@{You seem to have a missing or misspelled
  \expandafter\string\envir@end ...}%
  \envir@end
\fi}

\def\err@#1{\errmessage{Error: #1}}

\newhelp\defaulthelp@{Sorry, I already gave what help I could...^^J
Maybe you should try asking a human?^^J
An error might have occurred before I noticed any problems.^^J
``If all else fails, read the instructions.''}

\def\Err@{\errhelp\defaulthelp@\err@}

\def\Bibitem{\par\defaultreftexts\bibitem}
\def\RBibitem{\par\defaultrusreftexts\bibitem}

\AtBeginDocument{\def\refname{References}}
\AtBeginDocument{\def\bibname{References}}

\def\byfont{\rm}
\def\withfont{\rmfamily}
%\def\byfont{\slshape}
%\def\byfont{\itshape}
%   ®­¥æ ¬ ªà®á®¢ ¤«ï ®ä®à¬«¥­¨ï á¯¨áª  «¨â¥à âãàë
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% New commands for bibliography %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\@@ref{%
\ppunbox@\empty\empty\misc@box@\space%
\ppunbox@\empty\empty\bybox@\empty%
\ifbook@% Case 1: \book etc.
\ppunbox@{,}{ }\bookbox@\empty
\ppunbox@{,}{ }\bookinfobox@\empty
\ppunbox@{.}{ \bookvoltext@}\bookvolbox@\empty
\ppunbox@{:}{ \voltitletext@}\voltitlebox@\empty
\ppunbox@{,}{ }\procbox@\empty%
\ppunbox@{}{ (}\procinfobox@)%
\ppunbox@{,}{ }\serialbox@{}%
\ppunbox@{,}{ \voltext}\volbox@\empty
\ppunbox@,{ \volinfotext@ }\volinfobox@\empty
\ppunbox@,{ \serissuetext@ }\serissuebox@\empty
\ppunbox@,{ \issueinfotext@ }\issueinfobox@\empty
\ppunbox@{,}{ }\editionbox@ \empty%
\ppunbox@{,}{ \edtext~}\edbox@ \empty%
\ppunbox@{,}{ }\finalbookinfobox@\empty
\ppunbox@{,}{ }\publbox@ \empty
\ppunbox@{,}{ }\publaddrbox@{}%
\ppunbox@{;}{ }\publlbox@ \empty
\ppunbox@{,}{ }\publaddrrbox@{}%
\ppunbox@{;}{ }\publllbox@ \empty
\ppunbox@{,}{ }\publaddrrrbox@{}%
\ppunbox@,{ }\yrbox@{}%
\ppunbox@,{ \isbntext@ }\isbnbox@{}%
\else
\ifprocpaper@ % Case 2: \paper ... \inbook
\ifvoid \byybox@
\ppunbox@{,}{ ``}\paperbox@{''}%
\ppunbox@{,}{ }\paperinfobox@{}%
\else
\ppunbox@{,}{ ``}\paperbox@{''}%
\ppunbox@{,}{ }\paperinfobox@{}%
\ppunbox@{:}{ \byytext@ }\byybox@\empty%
\fi
\ppunbox@{,}{ \inbook@text }\bookbox@\empty
\ppunbox@{,}{ }\bookinfobox@\empty
\ppunbox@{.}{ \bookvoltext@}\bookvolbox@\empty
\ppunbox@{:}{ \voltitletext@}\voltitlebox@\empty
\ppunbox@{,}{ }\procbox@\empty%
\ppunbox@{}{ (}\procinfobox@)%
\ppunbox@{,}{ }\serialbox@{}%
\ppunbox@{,}{ \voltext}\volbox@\empty
\ppunbox@,{ \volinfotext@ }\volinfobox@\empty
\ppunbox@,{ \serissuetext@ }\serissuebox@\empty
\ppunbox@,{ \issueinfotext@ }\issueinfobox@\empty
\ppunbox@{,}{ }\editionbox@ \empty%
\ppunbox@{,}{ \edtext~}\edbox@ \empty%
\ppunbox@{,}{ }\finalbookinfobox@\empty
\ppunbox@{,}{ }\publbox@ \empty
\ppunbox@{,}{ }\publaddrbox@{}%
\ppunbox@{;}{ }\publlbox@ \empty
\ppunbox@{,}{ }\publaddrrbox@{}%
\ppunbox@{;}{ }\publllbox@ \empty
\ppunbox@{,}{ }\publaddrrrbox@{}%
\ifvoid \monthissuebox@
\ppunbox@,{ }\yrbox@{}%
\else
\ppunbox@,{ }\monthissuebox@\empty
\ppunbox@{}{ }\yrbox@{}%
\fi
\ppunbox@{,}{ \pagestext}\pagesbox@\empty
\ppunbox@,{ \isbntext@ }\isbnbox@{}%
\else % Case 3: \paper ... \jour
\ppunbox@{,}{ ``}\paperbox@{''}%
\ppunbox@{,}{ }\paperinfobox@{}%
\ppunbox@{,}{ \proc@text@}\procbox@{}%
\ppunbox@{}{ (}\procinfobox@)%
\ppunbox@{,}{ }\jourbox@{}%
\ifvoid\volbox@
\ppunbox@{,}{ }\yrbox@{}%
\ppunbox@{,}{ \volinfotext@}\volinfobox@\empty
\ppunbox@{,}{ \issuetext}\issuebox@\empty
\ppunbox@{,}{ \issueinfotext@}\issueinfobox@\empty
\else
\ppunbox@{,}{ \voltext}\volbox@\empty
\ppunbox@{,}{ \volinfotext@}\volinfobox@\empty
\ppunbox@:{}\issuebox@\empty
\ppunbox@{,}{ \issueinfotext@}\issueinfobox@\empty
\ifvoid \monthissuebox@
\ppunbox@{}{ (}\yrbox@{)}%
\else
\ppunbox@{}{ (}\monthissuebox@\empty
\ppunbox@{}{ }\yrbox@{)}%
\fi
\fi
\ppunbox@,{ \pagestext }\pagesbox@\empty
\ppunbox@,{ \paperidtext@ }\paperidbox@\empty
\fi
\fi
\ppunbox@\empty{ (}\miscnotebox@)%
\ppunbox@\empty{ \ (}\langbox@{)}%
\ppunbox@,{ }\totalpagesbox@{\totalpagestext@}%
\ppunbox@,{ \elinktext@ }\elinkbox@{}%
\ppunbox@,{ \arxivtext@ }\arxivbox@{}%
\ppunbox@{,}{ }\finalinfobox@\empty
\ppunbox@\empty{ (\withtext}\withbox@)%
\ppunbox@\empty{ }\@@finalinfobox@\empty
\if@misc@transl]\fi
\finalpunct
}%


%%%%%%%%%%%%%% ®¡ ¢«¥­¨¥ ®â ­®ï¡àï 2009 £®¤  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newbox\isbnbox@
\newbox\paperidbox@
\newbox\totalpagesbox@
\newbox\finalbookinfobox@
\newbox\volinfobox@
\newbox\issueinfobox@
\newbox\serissuebox@
\newbox\elinkbox@
\newbox\arxivbox@
\newbox\publlbox@
\newbox\publaddrrbox@
\newbox\publllbox@
\newbox\publaddrrrbox@
\newbox\byybox@
\newbox\monthissuebox@

\newbox\ptypebox@
\newbox\issnbox@
\newbox\journalnamebox@
\newbox\frombox@
\newbox\bibIDbox@
\newbox\citnumbox@
\newbox\citnumisibox@
\newbox\citnummsnbox@
\newbox\citnumelibbox@
\newbox\mainbox@
\newbox\sortdatebox@
\newbox\elibbox@
\newbox\scopusbox@
\newbox\Hrefsbox@

\newbox\editionbox@
\newbox\procbox@
\newbox\bookvolbox@
\newbox\voltitlebox@


\let\@@temp@@href=\href
\def\href#1#2{\@@temp@@href{#1}{{\tt #2}}}

%%%%   ¢ëå®¤¥ íâ¨å ª®¬ ­¤ - ­¨ç¥£® %%%%
\def\ptype{\makerefbox\ptypebox@\empty}
\def\issn{\makerefbox\issnbox@\empty}
\def\journalname{\makerefbox\journalnamebox@\empty}
\def\from{\makerefbox\frombox@\empty}
\def\bibID{\makerefbox\bibIDbox@\empty}
\def\citnum{\makerefbox\citnumbox@\empty}
\def\citnumisi{\makerefbox\citnumisibox@\empty}
\def\citnummsn{\makerefbox\citnummsnbox@\empty}
\def\citnumelib{\makerefbox\citnumelibbox@\empty}
\def\main{\makerefbox\mainbox@\empty}
\def\sortdate{\makerefbox\sortdatebox@\empty}
\def\elib{\makerefbox\elibbox@\empty}
%%%\def\scopus{\makerefbox\scopusbox@\empty}
\def\Hrefs{\makerefbox\Hrefsbox@\empty}

%%%%%%%%%%%%%%%%%%%%%%%%%%

\newif\if@finalpunct@
\@finalpunct@true
\def\isbn{\makerefbox\isbnbox@\empty}   \def\isbntext@{ISBN: }
\def\papernumber{\makerefbox\paperidbox@\empty}    \def\paperidtext@{}
%\let\paperid=\papernumber
\def\totalpages{\global\@finalpunct@false\makerefbox\totalpagesbox@\empty}
\def\byy{\makerefbox\byybox@\empty}

\def\finalbookinfo{\makerefbox\finalbookinfobox@\empty}
\def\edition{\makerefbox\editionbox@\empty}
\def\proc{\makerefbox\procbox@\empty}
\def\bookvol{\makerefbox\bookvolbox@\empty}
\let\bookvols=\bookvol
\def\voltitle{\makerefbox\voltitlebox@{\it}}
\def\volinfo{\makerefbox\volinfobox@\empty}   \def\volinfotext@{}
\def\issueinfo{\makerefbox\issueinfobox@\empty}
\def\serissue{\makerefbox\serissuebox@\empty}
\def\monthissue{\makerefbox\monthissuebox@\empty}   \def\monthissuetext@{}

\def\elink{\global\@finalpunct@true\makerefbox\elinkbox@\empty}    \def\elinktext@{}
\def\arxiv{\global\@finalpunct@true\makerefbox\arxivbox@\empty}    \def\arxivtext@{arXiv:\,\allowbreak}
%%%% ¥¯¥àì arxiv ¤«ï href-®¢ ­¨ï: %%%%%%%%%%%%%%%%%%%
%\def\hrarxiv#1{\edef\next{#1}\ifx\empty\next \ignorespaces\else\if@logos\if@finalinfo\@@finalinfo \@finalinfofalse\fi\href{#1}{\lower0.5mm\hbox{\includegraphics[height=3mm]{hrarxiv}}}\else\unskip\unskip\fi\fi}
\def\hrarxiv#1{\edef\next{#1}\ifx\empty\next \ignorespaces\else\if@logos\if@finalinfo\@@finalinfo \@finalinfofalse\fi\href{#1}{arXiv}\else\unskip\unskip\fi\fi}
%%% (¢â®à ï ¢¥àá¨ï - ¯®ª  ­¥â ª àâ¨­ª¨, â ¬ ¯à®áâ® ­ ¤¯¨áì arXiv:)
\def\finalinfo{\global\@finalpunct@true\makerefbox\finalinfobox@\empty}
\newbox\finalinfobox@
\def\@@finalinfo{\global\@finalpunct@true\makerefbox\@@finalinfobox@\empty}
\newbox\@@finalinfobox@


\def\publl{\makerefbox\publlbox@\empty}
\def\publaddrr{\makerefbox\publaddrrbox@\empty}
\def\publll{\makerefbox\publllbox@\empty}
\def\publaddrrr{\makerefbox\publaddrrrbox@\empty}



\def\defaultreftexts{\select@language{english}%
\color[rgb]{0,0,0}%
\frenchspacing
\gdef\edtext{ed.}\gdef\pagetext{}\gdef\pagestext{}%
\gdef\voltext{}\gdef\voltitletext@{}\def\bookvoltext@{V.\,}%
\gdef\issuetext{\No\,}\gdef\serissuetext@{no.\,}\gdef\t@appear{to appear}%
\def\eds{\gdef\edtext{eds.}\makerefbox\edbox@\empty}%
%\def\inbook@text{In:}}%
\def\issueinfotext@{}\def\byytext@{}\def\proc@text@{}%
\global\@finalpunct@true
\def\totalpagestext@{~pp.}%
\def\inbook@text{}\def\withtext{with }}%


\def\eds{\gdef\edtext{eds}\makerefbox\edbox@\empty}%

\def\defaultrusreftexts{\select@language{russian}%
\color[rgb]{0,0,0}%
\frenchspacing
\gdef\edtext{\cyrr\cyre\cyrd.}\gdef\pagestext{}%
\gdef\pagestext{}%
%\def\inbook@text{~á¡.:}% %\def\inbook@text{\CYRV~\cyrs\cyrb.}
\def\issueinfotext@{}\def\byytext@{}\def\proc@text@{}%
\def\inbook@text{}%
\global\@finalpunct@true
\def\totalpagestext@{~\cyrs.}%
\def\eds{\gdef\edtext{\cyrr\cyre\cyrd.}\makerefbox\edbox@\empty}%
\gdef\voltext{}\gdef\voltitletext@{}\def\bookvoltext@{\CYRT.\,}%
\gdef\issuetext{\No\,}\gdef\serissuetext@{\No\,}%
\gdef\t@appear{\cyrv~\cyrp\cyre \cyrch\cyra\cyrt\cyri}%
\def\withtext{\cyrs\cyro\cyrv\cyrm.\ \cyrs~}}%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% End of the new commands for bibliography %%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\href#1#2{#2}

\gdef\No{{\select@language{russian}\textnumero}}

\if@hyper
\RequirePackage[unicode]{hyperref}
\hypersetup{
colorlinks=true,
linkcolor=blue,
citecolor=blue,
urlcolor=blue,
filecolor=blue,
pdfpagemode=None,
pdfstartview=FitH,
pdfhighlight=/N
}
\fi



\newif\if@finalinfo
\@finalinfotrue

\def\Href@Crossref#1{\if@short
\href{http://dx.doi.org/#1}{\tt doi\,#1}\else
\href{#1}{\includegraphics[height=3mm]{crossref}}\fi}

\def\Href@Mathscinet#1{\if@short
\href{http://www.ams.org/mathscinet-getitem?mr=#1}{\tt MR\,#1}\else
\href{#1}{\includegraphics[height=3mm]{ams}}\fi
}

\def\Href@Mathnet#1{\if@short
\href{http://mi.mathnet.ru/#1}{\tt Mi\,#1}\else
\href{#1}{\includegraphics[height=3mm]{mi}}\fi
}

\def\Href@Zmath#1{\if@short
\href{http://www.zentralblatt-math.org/zmath/search/?an=#1}{\tt #1}\else
\href{#1}{\includegraphics[height=3mm]{zmath}}\fi
}

\def\Href@Ads#1{\if@short
\href{http://adsabs.harvard.edu/cgi-bin/bib_query?#1}{\tt ADS\,#1}\else
\href{#1}{\includegraphics[height=3mm]{ads}}\fi
}

%\def\crossref#1{\edef\next{#1}\ifx\empty\next \ignorespaces\else\if@finalinfo\@@finalinfo \@finalinfofalse\else\unskip, \fi\Href@Crossref{#1}\fi}
%\def\mathscinet#1{\edef\next{#1}\ifx\empty\next \ignorespaces\else\if@finalinfo\@@finalinfo \@finalinfofalse\else\unskip, \fi\Href@Mathscinet{#1}\fi}
%\def\mathnet#1{\edef\next{#1}\ifx\empty\next \ignorespaces\else\if@finalinfo\@@finalinfo \@finalinfofalse\else\unskip, \fi\Href@Mathscinet{#1}\fi}
%\def\zmath#1{\edef\next{#1}\ifx\empty\next \ignorespaces\else\if@finalinfo\@@finalinfo \@finalinfofalse\else\unskip, \fi\Href@Zmath{#1}\fi}
%\def\adsnasa#1{\edef\next{#1}\ifx\empty\next \ignorespaces\else\if@finalinfo\@@finalinfo \@finalinfofalse\else\unskip, \fi\Href@Ads{#1}\fi}


\def\crossref#1{\edef\next{#1}\ifx\empty\next \ignorespaces\else\if@logos\if@finalinfo\@@finalinfo \@finalinfofalse\fi\href{#1}{\includegraphics[height=3mm]{crossref}}\else\unskip\unskip\fi\fi}
\def\mathscinet#1{\edef\next{#1}\ifx\empty\next \ignorespaces\else\if@logos\if@finalinfo\@@finalinfo \@finalinfofalse\fi\href{#1}{\includegraphics[height=3mm]{ams}}\else\unskip\unskip\fi\fi}
\def\mathnet#1{\edef\next{#1}\ifx\empty\next \ignorespaces\else\if@logos\if@finalinfo\@@finalinfo \@finalinfofalse\fi\href{#1}{\includegraphics[height=3mm]{mi}}\else\unskip\unskip\fi\fi}
\def\zmath#1{\edef\next{#1}\ifx\empty\next  \ignorespaces\else\if@logos\if@finalinfo\@@finalinfo \@finalinfofalse\fi\href{#1}{\includegraphics[height=3mm]{zmath}}\else\unskip\unskip\fi\fi}
\def\adsnasa#1{\edef\next{#1}\ifx\empty\next  \ignorespaces\else\if@logos\if@finalinfo\@@finalinfo \@finalinfofalse\fi\href{#1}{\includegraphics[height=3mm]{ads}}\else\unskip\unskip\fi\fi}
\def\isi#1{\edef\next{#1}\ifx\empty\next  \ignorespaces\else\if@logos\if@finalinfo\@@finalinfo \@finalinfofalse\fi\href{#1}{\lower 0.7mm\hbox{\includegraphics[height=3mm]{isi}}}\else\unskip\unskip\fi\fi}
\def\scopus#1{\edef\next{#1}\ifx\empty\next  \ignorespaces\else\if@logos\if@finalinfo\@@finalinfo \@finalinfofalse\fi\href{#1}{\lower 0.1mm\hbox{\includegraphics[height=3mm]{scopus}}}\else\unskip\unskip\fi\fi}


\def\@Color{\if@hyper\color[rgb]{0,0,1}\fi}

\def\@No@Color{\color[rgb]{0,0,0}}

\long\def\@makefntext#1{\@No@Color\parindent 12pt%\noindent
 $^{\@thefnmark}$#1}

\def\thefootnote{\@No@Color\ifnum\c@footnote>0 \arabic{footnote}\else\fi}

\def\footnoterule{\@No@Color\kern-3\p@
  \hrule \@width 2in \kern 2.6\p@} % the \hrule is .4pt high

%\def\thepage{\@No@Color\arabic{page}}

\defaultreftexts

\endinput
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

